IntereStyle: Encoding an Interest Region for Robust StyleGAN Inversion

Recently, manipulation of real-world images has been highly elaborated along with the development of Generative Adversarial Networks (GANs) and corresponding encoders, which embed real-world images into the latent space. However, designing encoders of GAN still remains a challenging task due to the trade-off between distortion and perception. In this paper, we point out that the existing encoders try to lower the distortion not only on the interest region, e.g., human facial region but also on the uninterest region, e.g., background patterns and obstacles. However, most uninterest regions in real-world images are located at out-of-distribution (OOD), which are infeasible to be ideally reconstructed by generative models. Moreover, we empirically find that the uninterest region overlapped with the interest region can mangle the original feature of the interest region, e.g., a microphone overlapped with a facial region is inverted into the white beard. As a result, lowering the distortion of the whole image while maintaining the perceptual quality is very challenging. To overcome this trade-off, we propose a simple yet effective encoder training scheme, coined IntereStyle, which facilitates encoding by focusing on the interest region. IntereStyle steers the encoder to disentangle the encodings of the interest and uninterest regions. To this end, we filter the information of the uninterest region iteratively to regulate the negative impact of the uninterest region. We demonstrate that IntereStyle achieves both lower distortion and higher perceptual quality compared to the existing state-of-the-art encoders. Especially, our model robustly conserves features of the original images, which shows the robust image editing and style mixing results. We will release our code with the pre-trained model after the review.

==> fig/edit_app.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=.99\textwidth]{figures/edit_app.pdf}
\end{center}
\caption{
% 
\textbf{Editing comparison.}
Edited images via latent manipulations through various encoders. We find our model robustly edits the images even in the hard cases, \eg, obstacles on the face, shadows, while other models occur severe artifacts. Especially, models that show low distortion on the inversion, \eg, pSp, and $\text{Restyle}_{pSp}$, show bad editability on the various editing directions.
% Best viewed in zoom-in.
}
\label{fig:edit_app}
\end{figure*}

==> fig/interpolation_app.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\textwidth]{figures/interpolation_app.pdf}
\end{center}
\caption{
% 
\textbf{Latent interpolation.} Additional latent interpolation results, compared to $\text{Restyle}_{pSp}$. All the images are randomly selected from CelebA-HQ test dataset. Best viewed in zoom-in.
}
\label{fig:interpolation_app}
\end{figure*}

==> fig/interpolation_app_magnify.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\textwidth]{figures/figure1_app.pdf}
\end{center}
\caption{
% 
\textbf{Latent interpolation.} Comparison of interpolation results between our model and existing state-of-the-art model, $\text{Restyle}_{pSp}$. We show the magnified results of the most interest region, \eg, eyes, nose, and mouth. In $\text{Restyle}_{pSp}$, undesirable extension of pupils and distortion and nostrils and teeth. In contrast, our model consistently generates stable images without severe distortion.
}
\label{fig:interpolation_app_magnify}
\end{figure*}

==> fig/inversion_app.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\textwidth]{figures/inversion.pdf}
\end{center}
\caption{
% 
\textbf{Various inversion results.} Various inversion results of our model. We plot the inversion images along with the intermediate outputs during iterative iteration. All images are sampled from CelebA-HQ test dataset.
}
\label{fig:inversion_app}
\end{figure*}

==> fig/preprocess_app.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=.99\textwidth]{figures/preprocess.pdf}
\end{center}
\caption{
% 
\textbf{Preprocessing.}
Preprocessed images using uninterest filter for training. In the uninterest region, we blur severely at the beginning of the iteration, as shown in $I_{1}$ and $I_{2}$. Gradually, images get clear, and we use the image at the last iteration, $I_{4}$, becomes same with $I$.
% Best viewed in zoom-in.
}
\label{fig:preprocess_app}
\end{figure*}
